Planning with Linear Temporal Logic Specifications: Handling Quantifiable and Unquantifiable Uncertainty

This work studies the planning problem for robotic systems under both quantifiable and unquantifiable uncertainty. The objective is to enable the robotic systems to optimally fulfill high-level tasks specified by Linear Temporal Logic (LTL) formulas. To capture both types of uncertainty in a unified modelling framework, we utilise Markov Decision Processes with Set-valued Transitions (MDPSTs). We introduce a novel solution technique for the optimal robust strategy synthesis of MDPSTs with LTL specifications. To improve efficiency, our work leverages limit-deterministic B\"uchi automata (LDBAs) as the automaton representation for LTL to take advantage of their efficient constructions. To tackle the inherent nondeterminism in MDPSTs, which presents a significant challenge for reducing the LTL planning problem to a reachability problem, we introduce the concept of a Winning Region (WR) for MDPSTs. Additionally, we propose an algorithm for computing the WR over the product of the MDPST and the LDBA. Finally, a robust value iteration algorithm is invoked to solve the reachability problem. We validate the effectiveness of our approach through a case study involving a mobile robot operating in the hexagonal world, demonstrating promising efficiency gains.

==> settings.tex <==
\usepackage[
	citestyle=ieee, 
    bibstyle=ieee,
    style=numeric-comp,
    sorting=nty,
    maxbibnames=99, % Make sure we are printing all authors in the appendix
    ]{biblatex}
    
% Makes the last name first in the bibliography.
% \DeclareNameAlias{author}{last-first}
\DeclareNameAlias{author}{family-given}
    
% Specify the margins. This is 6.25inches in text with which 
% can be used to size figures to the correct size.
\usepackage[a4paper, margin=2.5625cm]{geometry}

\usepackage{eso-pic}					% Packages for layout and graphics 
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{fadings}
\usepackage{setspace}
% \usepackage{tocloft}		 			% Fixing a bug with page style changes for toc
% \tocloftpagestyle{plain}
\usepackage{etoc} 						% Separate tocs for appendix and the rest    
\usepackage{chngcntr}					% Count figures within chapters
\usepackage{booktabs}					% Table formatting
\usepackage{fancyhdr}					% Setting the style for header and footer.
\usepackage{tabularx}
\usepackage{multirow}                   % For better tables 
\usepackage[hidelinks]{hyperref}		% Clickable links
\usepackage{nameref}					% References with names
\usepackage[parfill]{parskip}			% New line instead of indent for sections
\usepackage{tcolorbox}					% Create boxes around content
\tcbset{colback=white,arc=0mm}

\usepackage[english]{babel}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathdots}
\usepackage{yhmath}
\usepackage{siunitx}
\usepackage{array}
\usepackage{gensymb}
\usepackage{amssymb}
\usepackage{mathtools}  

% New packages
%\usepackage[table]{xcolor}
%\usepackage{array}
%\usepackage{makecell}
%\usepackage{subcaption}
%\usepackage{placeins}


% Add text to math arrows.

\usepackage{cancel}
\usepackage{color}
\usepackage{multirow}
\usepackage{textcomp}               % Fixing warning for gensyb \perthousand
\usepackage{svg}                    % including svg files
\usepackage{caption}                % For subfigures
\usepackage{subcaption}
%\usepackage{fontspec}
\usepackage{sectsty}
\usepackage{tocloft}

\usepackage[printonlyused]{acronym}


\counterwithin{figure}{section} 
\counterwithin{table}{section}

% % Specifying fonts
% \setmainfont{Georgia} 
% \setsansfont{Arial}
% \newfontfamily\footerfont{Georgia}

\chapterfont{\sffamily\fontsize{17}{17}}
\sectionfont{\sffamily\fontsize{14}{15}}
\subsectionfont{\sffamily\fontsize{13}{15}}
\subsubsectionfont{\sffamily\fontsize{12}{15}}

% Remove the title and make sure that the text is adjusted
% \usepackage{abstract}
% \setlength{\absleftindent}{0mm}
% \renewcommand{\abstractname}{\vspace{-\baselineskip}}
% \renewcommand{\abstractnamefont}{\sffamily\fontsize{14}{15}}
% \renewcommand{\abstracttextfont}{\normalfont\fontsize{12}{13}}

% Renaming and setting style of table of contents
\renewcommand*\contentsname{Contents}
\renewcommand*\cfttoctitlefont{\fontsize{16}{0}\bf\sffamily}
\renewcommand\cftchapfont{\fontsize{14}{0}\bf\sffamily}
\renewcommand\cftchappagefont{\fontsize{13}{0}\bf\sffamily}
\renewcommand\cftsecfont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsecpagefont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsubsecfont{\fontsize{12}{0}\sffamily}
\renewcommand\cftsubsecpagefont{\fontsize{12}{0}\sffamily}

% Styling the header and footer
\fancyhf{}
\fancyhead{}
\fancyfoot{}
\fancyhead[L]{\fontsize{11}{10}\selectfont\leftmark}
\fancyfoot[R]{\footerfont\thepage}
\setlength{\headheight}{15.5pt}


\fancypagestyle{plain}{
    \fancyhf{}
    \fancyhead{}
    \fancyfoot{}
    \renewcommand{\headrulewidth}{0pt}
    \fancyfoot[R]{\footerfont\thepage}
}

\pagestyle{fancy}

% Making the command for placing text in random locations
\newcommand\PlaceText[3]{%
\begin{tikzpicture}[remember picture,overlay]
\node[outer sep=0pt,inner sep=0pt,anchor=south west] 
  at ([xshift=#1,yshift=-#2]current page.north west) {#3};
\end{tikzpicture}%
}

% Disable hyphenation
\pretolerance=10000
\tolerance=2000 
\emergencystretch=50pt

